X-Light: Cross-City Traffic Signal Control Using Transformer on Transformer as Meta Multi-Agent Reinforcement Learner

The effectiveness of traffic light control has been significantly improved by current reinforcement learning-based approaches via better cooperation among multiple traffic lights. However, a persisting issue remains: how to obtain a multi-agent traffic signal control algorithm with remarkable transferability across diverse cities? In this paper, we propose a Transformer on Transformer (TonT) model for cross-city meta multi-agent traffic signal control, named as X-Light: We input the full Markov Decision Process trajectories, and the Lower Transformer aggregates the states, actions, rewards among the target intersection and its neighbors within a city, and the Upper Transformer learns the general decision trajectories across different cities. This dual-level approach bolsters the model's robust generalization and transferability. Notably, when directly transferring to unseen scenarios, ours surpasses all baseline methods with +7.91% on average, and even +16.3% in some cases, yielding the best results.

==> 3-pro_setup.tex <==
% \section{Problem Statement} \label{sub Problem Statement}
%Our goal is to build a general multi-agent TSC method that can easily transfer new intersections or scenarios. Therefore, we define this problem as the Meta-RL for multiple intersection collaboration. We consider the traffic signal control on different scenarios/intersections as different meta-tasks. Our method needs to be able to achieve better performance in a variety of intersections or scenarios, even if these intersections or scenarios have never been encountered before. As shown in Figure~\ref{fig: Preliminary3}, different trajectories represent different intersections and tasks, and the trajectories within the same color surface indicate they are in the same scenario. $\phi$ is the history embedding space. One goal of our method is to learn $\phi$ to make a distinction among the tasks in the embedding space $\phi$, and minimize loss across different tasks:
%\begin{equation}
%    \theta = \arg\min_{\theta} \frac{1}{m}\sum_{i=1}^m\mathcal{L}(f_{\theta}(I_i), I_i),
%\end{equation}
%where $\theta$ is the policy parameter; $f_{\theta}(I_i)$ is the policy output, which denotes the policy to solve the task $I_i$; $\mathcal{L}$ is the loss, which we will show in the section~\ref{subsection Detailed training settings}.


% Besides this, we also define the problem of multi-agent traffic signal control in different scenarios as multi-agent Markov decision processes (MMDPs)~\cite{boutilier1996planning}, each agent controls an intersection, and each agent observes part of the total system condition which only includes the transition information of the target intersection and its top $n$ nearest neighbor intersection. We can represent this as $\langle \mathcal{S},\mathcal{O},\mathcal{A},\mathcal{P}, r,\gamma \rangle$.  
% \textcolor{red}{
% We define the problem of multi-agent traffic signal control in different scenarios as Meta-RL partially observed Markov decision processes (Meta-RL POMDPs)~\cite{humplik2019meta}. Given a set of scenarios $\mathcal{X}$ sampled over task distribution $\varepsilon$. Each agent controls one of the intersections $I_i$ from scenarios, and each intersection has its neighboring intersections $\textit{\textbf{I}}_{\mathcal{N}}$, where $\mathcal{N}=\{\mathcal{N}_1,\ldots,\mathcal{N}_n\}$. Each agent observes part of the total system condition which only includes the transition information of the target intersection $i$ and its top $n$ nearest neighbor intersection. We can represent this as $\langle \mathcal{S},\mathcal{O},\mathcal{A},\mathcal{P}, r,\gamma \rangle$. $\mathcal{S}$ is the state space, and $s_t \in \mathcal{S}$ denotes the state at time step t. Since the environment is partially observed, each agent only has access to its local observation: $o_t^i$ and $o_t^{\mathcal{N}_1,...,\mathcal{N}_n}$. The observation is acquired through an observation function $D(s): \mathcal{S} \rightarrow \mathcal{O}$. At time step $t$, each agent takes an action to perform a joint action $\textbf{a}$ and cause the state transition $\mathcal{P}(s_{t+1}|s_t, \textbf{a}) := \mathcal{S} \times \mathcal{A}^N \rightarrow \mathcal{S}$ and agent $i$ received a reward $r_t^i$. When optimizing, we want to maximize cumulative reward: $\sum_t\gamma^tr_t^i$, where $\gamma$ is the discounted factor.}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.95\textwidth]{FormattingGuidelines-IJCAI-24/figs/main_fig_v6.pdf} % Reduce the figure size so that it is slightly narrower than the column.
% \caption{Network design in our framework. \hua{needs explanation to correspond to Section 4.1}}
% \label{fig: method}
% \end{figure*}


% \textcolor{red}{
% In meta-reinforcement learning, we need to be able to achieve great performance in a variety of intersections or scenarios, even if these intersections or scenarios have never been encountered before. As shown in Figure~\ref{fig: intro}, different surfaces represent different tasks, one goal is to learn $\theta$ to make a distinction among the tasks in the embedding space $\theta$, and minimize loss across different tasks:
% \begin{equation}
%    \theta = \arg\min_{\theta} \frac{1}{m}\sum_{i=1}^m\mathcal{L}(f_{\theta}(I_i), I_i),
% \end{equation}
% where $\theta$ is the policy parameter; $f_{\theta}(I_i)$ is the policy output, which denotes the policy to solve the task $I_i$; $\mathcal{L}$ is the loss.}

% \begin{itemize}
% % \item State space $\mathcal{S}$ and observation space $\mathcal{O}$. We assume 
% % %an environment has N intersections, and 
% % the agent $i$ can observe part of the environment state space $s_t \in \mathcal{S}$ at time step $t$, as its observation $o_t^i \in \mathcal{O}$.
% \item We choose five features from the observations as states: queue length, current phase, occupancy, flow, and the number of cars that are stopping~\cite{wei2021recent}.
% \item Set of actions $\mathcal{A}$. At each time step $t$, the agent $i$ can choose action $a_t^i$ from available action set $\mathcal{A}^i$, in the next $\Delta t$ seconds. In our experiments, we set $\Delta t$ as 15 seconds.
% %\item The state transition probability $\mathcal{P}$. At timestep $t$, all agents do joint action $\textbf{a}=\{a_t^1,\ldots, a_t^N\}$, making the state transition to $s_{t+1}$. The state transition dynamic can be formulated as $\mathcal{P}(s_{t+1}|s_t, \textbf{a}):\mathcal{S}\times\mathcal{A}^N \rightarrow \mathcal{S}$.
% \item 
% % Reward $r$. Each agent $i$ can receive an immediate reward $r_t^i$ at time step $t$. When optimizing, we want to maximize cumulative reward: $\sum_t\gamma^tr_t^i$, where $\gamma$ is the discounted factor. 
% We define the reward $r$ as the weighted average of queue length, wait time, delay time, and pressure. The detailed setting is recorded in Appendix~\ref{sub Implementation details}.

% \end{itemize}
